Modular Analysis of Distributed Hybrid Systems using Post-Regions (Full Version)

We introduce a new approach to analyze distributed hybrid systems by a generalization of rely-guarantee reasoning. First, we give a system for deductive verification of class invariants and method contracts in object-oriented distributed hybrid systems. In a hybrid setting, the object invariant must not only be the post-condition of a method, but also has to hold in the post-region of a method. The post-region describes all reachable states after method termination before another process is guaranteed to run. The system naturally generalizes rely-guarantee reasoning of discrete object-oriented languages to hybrid systems and carries over its modularity to hybrid systems: Only one dL-proof obligation is generated per method. The post-region can be approximated using lightweight analyses and we give a general notion of soundness for such analyses. Post-region based verification is implemented for the Hybrid Active Object language HABS.

==> ddl.tex <==
We briefly review \emph{differential dynamic logic} (\ddl)
\cite{DBLP:journals/jar/Platzer17,Platzer18} as implemented in the
interactive theorem prover \KeYmaeraX\ \cite{FultonMQVP15}.
%
Differential dynamic logic expresses the combined discrete and
continuous dynamics of hybrid systems in a sequential imperative
programming language called \emph{hybrid programs}.  Its syntax and
informal semantics are in Table~\ref{tab:hybrid-programs}.

\begin{table}[htb]
\centering
\caption{Hybrid programs in \ddl}
\label{tab:hybrid-programs}
\begin{tabular}{ll}
Program & Informal semantics   \\\hline
$\ptest{\phi}$         & Test whether formula $\phi$ is true, abort if false\\
$\pumod{x}{\theta}$    & Assign value of term $\theta$ to variable $x$\\
$\prandom{x}$          & Assign any (real) value to variable $x$\\
$\pevolvein{\D{x}=\theta}{H}$& Evolve ODE $\D{x} = \theta$ for any duration $t{\geq}0$ \\
& with evolution domain constraint $H$ true throughout\\
$\alpha;\beta$         & Run $\alpha$ followed by $\beta$ on resulting state(s)\\
$\alpha\cup\beta$      & Run either $\alpha$ or $\beta$ non-deterministically\\
$\prepeat{\alpha}$     & Repeat $\alpha$ $n$ times, for any $n\in\mathbb{N}$
\end{tabular}
\end{table}

Hybrid programs provide the usual discrete statements: assignment
($\pumod{x}{\theta}$), non-deterministic assignment ($\prandom{x}$),
test ($\ptest{\phi}$), non-deterministic choice ($\alpha\cup\beta$),
sequential composition ($\alpha ; \beta$), and non-deterministic
repetition ($\prepeat{\alpha}$).  A typical modeling pattern combines
non-deterministic assignment and test (e.g., ``$\prandom{x};\ptest{H}$'')
to choose any value subject to a Boolean constraint
$H$.  Standard control structures are expressible, for example:
\begin{inparaenum}[(i)]
\item
  $\kyx{if}~ H ~\kyx{then}~ \alpha ~\kyx{else}~ \beta \equiv
  \pchoice{(\ptest{H};\alpha)}{(\ptest{\lnot H};\beta)}$,
\item
  $\kyx{if}~ H ~\kyx{then}~ \alpha \equiv
  \pchoice{(\ptest{H};\alpha)}{(\ptest{\lnot H})}$,
\item
  $\kyx{while}~(H) ~\alpha \equiv
  \prepeat{(\ptest{H};\alpha)};\ptest{\lnot H}$.
\end{inparaenum}

For continuous dynamics, the notation $\pevolvein{\D{x} = \theta}{H}$
represents an ordinary differential equation (ODE) system (derivative
$\D{x}$ in time) of the form $\D{x}_1 = \theta_1$, \dots,
$\D{x}_n = \theta_n$.  Any behavior described by the ODE stays inside
the evolution domain $H$, i.e.\ the ODE is followed for a
non-deterministic, non-negative period of time, but stops before $H$
becomes false.  For example, a basic model of the water level $x$ in a
tank draining with flow $-f$ is given by the ODE
$\pevolvein{\D{x}=-f}{x \geq 0}$, where the evolution domain
constraint $x \geq 0$ means the tank will not drain to negative water
levels.
% \ektodo{Maybe another example so the reader doesn't confuse it with
% the following water tanks?}
With a careful modeling pattern, continuous behavior can be governed by $H$ so that one can react to
events, but it is not otherwise restricted or influenced: The pattern
$\pchoice{\pevolvein{\D{x} = \theta}{H}}{\pevolvein{\D{x} =
    \theta}{\widetilde{H}}}$ permits control intervention to achieve
different behavior triggered by an event.  $\widetilde{H}$ is the weak
complement of~$H$: they share exactly their \emph{boundary} from which both
behaviors are possible. For example, $H\equiv x\leq 0$,
$\widetilde{H}\equiv x\geq 0$.

The \dL-formulas $\phi,\,\psi$ relevant for this paper are
propositional logic operators $\phi\land\psi$, $\phi\lor\psi$,
$\phi\limply\psi$, $\neg\phi$ and
%$\forall{x}{~\phi}$, and $\exists{x}{~\phi}$ 
comparison expressions $\theta\sim\eta$, where
$\sim\mathop{\in}\{<,\,\leq,\,=,\,\neq,\,\geq,\,>\}$ and
$\theta,\,\eta$ are real-valued terms over $\{+,\,-,\,\cdot\,,/\}$. In
addition, there is the \dL\ modal operator $\dbox{\alpha}{\phi}$.
\iffalse
%
\begin{equation*}
  \phi,\psi ::= \phi\land\psi\ |\ \phi\lor\psi\ |\ \phi\limply\psi\ |\ \neg\phi\ |\ \theta \sim \eta
  % |\ \forall{x}{~\phi}\ |\ \exists{x}{~\phi}\ 
  |\ \dbox{\alpha}{\phi}\
\end{equation*}
%
\fi
%
The \dL-formula $\dbox{\alpha}{\phi}$ is true iff $\phi$ holds in all
states reachable by program $\alpha$.
%
The formal semantics of $\dL$
\cite{DBLP:journals/jar/Platzer17,Platzer18} is a Kripke semantics in
which the states of the Kripke model are the states of the hybrid
system.
% States are maps $\nu:\allvars\to\reals$ assigning a real value
% $\nu(x)$ to each variable $x\in\allvars$.
The semantics of a hybrid program $\alpha$ is a relation
$\llbracket\alpha\rrbracket$ between its initial and final states.
Specifically, $\nu\models\dbox{\alpha}\phi$ iff $\omega\models\phi$
for all states $(\nu,\omega) \in \llbracket\alpha\rrbracket$, so all
runs of $\alpha$ from $\nu$ are safe relative to $\phi$.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

